A Policy Optimization Method Towards Optimal-time Stability

In current model-free reinforcement learning (RL) algorithms, stability criteria based on sampling methods are commonly utilized to guide policy optimization. However, these criteria only guarantee the infinite-time convergence of the system's state to an equilibrium point, which leads to sub-optimality of the policy. In this paper, we propose a policy optimization technique incorporating sampling-based Lyapunov stability. Our approach enables the system's state to reach an equilibrium point within an optimal time and maintain stability thereafter, referred to as "optimal-time stability". To achieve this, we integrate the optimization method into the Actor-Critic framework, resulting in the development of the Adaptive Lyapunov-based Actor-Critic (ALAC) algorithm. Through evaluations conducted on ten robotic tasks, our approach outperforms previous studies significantly, effectively guiding the system to generate stable patterns.

==> corl/backup/sec1_intro.tex <==

\begin{wrapfigure}{r}{7cm}
\vspace{-20pt}
\begin{center}
\includegraphics[width=0.4\textwidth]{corl/figures/intro.pdf}
\end{center}
\caption{\small Intuitive example showing the mean cost stability. The figure shows the relationship between three sets, like the whole state space, $\{s \mid c_\pi(s) \leq b\}$  and $\{s \mid c_\pi(s) = 0\}$. The red line represents a diverging trajectory. The yellow line represents a trajectory without stability. The trajectories coloured cyan and purple remain stable, whereas the state in the purple trajectory reaches the set $\{s \mid c_\pi(s) = 0\}$ more quickly. The task aims to obtain the policy that can generate the purple trajectory.}
\label{figure:intro}
\vspace{-10pt}
\end{wrapfigure}

Reinforcement learning (RL) controllers have achieved excellent performance in a large variety of robotic tasks \citep{hwangbo2019learning,andrychowicz2020learning}. However, a lack of stability in current methods introduces additional risks to the robots and environments, especially when there exist some external disturbances \citep{jin2020neural}. Thus, maintaining the system's stability remains an essential requirement in RL-based methods.

% In control-theoretic methods, the existence of a Lyapunov function can be represented as a sign of stability. But how to find a Lyapunov function remains an open challenge in the non-linear dynamic system \citep{la2012stability}. 

% Lyapunov functions can be designed for a linear system with specific criteria in the form of a quadratic positive-definite function.
% Stability is a crucial notion of safety, whose violation can cause unsafe behaviours \citep{jin2020neural}. 


In control-theoretic methods, the presence of a Lyapunov function can be represented as a sign of stability \citep{la2012stability} (More details see Appendix \ref{app:Lya}). Thus, RL researchers trained the neural Lyapunov network to search for a feasible Lyapunov function for the system. For the model-based setting, the discrete-time Lyapunov's second method (Appendix \ref{app:Lya}) is suitable because the difference of Lyapunov function can be obtained by the dynamic model \citep{berkenkamp2017safe,richards2018lyapunov,gaby2021lyapunov,zhou2022neural}. However, the discrete stability condition is not satisfied everywhere in model-free methods. This is because the difference of Lyapunov function $V(s_{t+1})- V(s_t)$ is not accurate when $s_{t+1}$ is randomly sampled. Therefore, it is not reasonable that prior studies added discrete-time Lyapunov constraints into the objective function directly \citep{chang2021stabilizing,xiong2022model}. 
Taking the drawback into account, the Lyapunov-based Actor-Critic (LAC) algorithm was developed to achieve sampling-based stability \citep{han2020actor, han2021reinforcement, zhao2021neural}. The mean cost stability they proposed maintains the system's state to behave stable around an equilibrium point. Despite the great success (The related work part is provided in Appendix \ref{app:related}.), their method can not guarantee that the optimal policy makes the state converge to the equilibrium point as quickly as possible. To better understand the importance of the demand, we give an intuitive example of the optimality and stability we introduced in Figure \ref{figure:intro}. To recap, it remains a challenge reaching stable regions most quickly and then behaving stable in model-free RL methods. 


To address the above problem, we demonstrate the sampling-based Lyapunov stability we propose can maintain the stability condition in Definition \ref{MSS}. Furthermore, we construct a heuristic-based policy optimization, which facilitates the policy to find the optimal point heuristically without violating the stability condition. According to the policy optimization method, we build the Adaptive Lyapunov-based Actor-Critic algorithm (ALAC) to reach the stability of the system as quickly as possible. 
% Due to the introduction of a Lyapunov candidate and the Lagrangian-based policy optimization, our method mitigates the coupling relationship between various constraints and the objective function compared with previous studies. 
Experiments show that our method provides promising results under stability constraints on some robotic control problems, like walking of legged robots, trajectory planning of a free-floating space robot, and so on. Another interesting finding is that, in contrast to traditional RL algorithms, our method facilitates the controller to enhance the robustness and generalization of the whole system \footnote{See our project page at \href{https://sites.google.com/view/adaptive-lyapunov-actor-critic}{https://sites.google.com/view/adaptive-lyapunov-actor-critic}.}. 








% ==================================================================================


% To better improve the current research, we hope the Lyapunov-based constraint can facilitate the policy to reach the optima within the set of sampling-based stability. To better understand the principle, we give an intuitive example in Figure \ref{figure:intro}.


% Thanks to the emergence of deep learning, researchers noticed that the neural Lyapunov function had an outperforming representation ability, thereby making it possible to search for a feasible Lyapunov function. According to Lyapunov's second method for stability, the neural Lyapunov function is trained by forcing the updating direction toward decreasing the Lyapunov function along an episode's state trajectories \citep{chang2019neural}. In the early stage of time, these methods are only suitable for the model-based setting because the difference of Lyapunov function with respect to time brings a requirement of dynamic model \citep{berkenkamp2017safe,richards2018lyapunov}. In contrast to model-based methods, model-free reinforcement learning methods have achieved superior performance on many complex robotic systems \citep{hwangbo2019learning,andrychowicz2020learning}. Therefore, researchers proposed some methods to overcome the above issue. Firstly, they applied the discrete Lyapunov stability condition directly in the optimization. Then, the Lyapunov conditions can be viewed as multiple constraints. Prior studies added those constraints into the objective function. Specifically, the objective function enables the system to reach optimality and stability together. (The related work part is provided in Appendix \ref{app:related}.) 

% Admittedly, RL-based approaches with the help of the Lyapunov function achieve promising performance. However, the discrete Lyapunov stability condition should be satisfied in the whole state space, which means infinity constraints for continuous control tasks. Due to the sampling-based optimization in RL, current approaches sample some data pairs randomly, which causes a serious problem that the discrete stability condition is not convincing. Furthermore, reaching optimality and stability together remains a challenge for their objective function. Because the Lyapunov stability condition introduces various constraints in the objective function, it is hard to balance the optimality and stability of the system. In practical experiments, we find that previous constraints are either loose to find ineffective Lyapunov functions or tight to make the policy trapped into a sub-optimal point. Therefore, to better improve the current research, we hope the Lyapunov-based constraint can facilitate the policy to reach the optima within the set of the sampling-based stability. To better understand the principle, we give an intuitive example in Figure \ref{figure:intro}.


% To address the above issues, we propose the Adaptive Lyapunov-based Actor-Critic algorithm (ALAC). Unlike the discrete Lyapunov stability condition, we propose a novel sampling-based stability condition called Adaptive Stability Certification (ASCO). Meanwhile, ASCO can guide the policy to search for the optimal point heuristically. Thus, based on the ASCO condition, we design the Adaptive Lyapunov-based Actor-Critic algorithm (ALAC) to reach the optimality and stability of the system. Due to the introduction of a Lyapunov candidate and the Lagrangian-based policy optimization, our method eliminates the coupling relationship between various constraints and the objective function. Experiments show that our method provides promising results under stability constraints on some robotic control problems, like walking of legged robots, trajectory planning of a free-floating space robot, and so on. Another interesting finding is that, in contrast to traditional RL algorithms, our method facilitates the controller to enhance the robustness, generalization, and efficiency of the whole system \footnote{See our project page at https://sites.google.com/view/adaptive- lyapunov-actor-critic.}. 

% Our contributions are the following:

% \begin{itemize}
%     \item we propose a Heuristic Lyapunov Certification, which meets the sampling-based stability of mean cost. Moreover, it guides the current policy to approaches to the optimal point adaptively in the context of classical feedback control.
%     \item we design a Heuristic  Lyapunov-based Actor-Critic algorithm combined the above certification with a contrained Lyapunov network. Interestingly, we also propose an Lagrangian-based optimization method to update the parameters of the Heuristic Lyapunov Certification.
%     \item our method outperforms other baselines on diverse robotic tasks with two metrics, constraint violations and mean costs. Furthermore, the controller trained by our method achieves higher generalization ability compared with the method without the stability guarantee. 
% \end{itemize}


%%SL.1.17: Don't forget to fill in the citations...

